Designing Biological Sequences via Meta-Reinforcement Learning and Bayesian Optimization

The ability to accelerate the design of biological sequences can have a substantial impact on the progress of the medical field. The problem can be framed as a global optimization problem where the objective is an expensive black-box function such that we can query large batches restricted with a limitation of a low number of rounds. Bayesian Optimization is a principled method for tackling this problem. However, the astronomically large state space of biological sequences renders brute-force iterating over all possible sequences infeasible. In this paper, we propose MetaRLBO where we train an autoregressive generative model via Meta-Reinforcement Learning to propose promising sequences for selection via Bayesian Optimization. We pose this problem as that of finding an optimal policy over a distribution of MDPs induced by sampling subsets of the data acquired in the previous rounds. Our in-silico experiments show that meta-learning over such ensembles provides robustness against reward misspecification and achieves competitive results compared to existing strong baselines.

==> imgs/AMP_multiround.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
title={AMP Task},
x grid style={white!69.0196078431373!black},
xlabel={Number of samples},
xmin=112.5, xmax=3137.5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cumulative maximum},
ymin=0.137680158222965, ymax=0.928574110106748,
ytick style={color=black}
]
\path [fill=color0, fill opacity=0.2]
(axis cs:250,0.346614454193629)
--(axis cs:250,0.325885545210325)
--(axis cs:500,0.350322923474925)
--(axis cs:750,0.379211648715696)
--(axis cs:1000,0.525791697478316)
--(axis cs:1250,0.725104412697482)
--(axis cs:1500,0.750261561365755)
--(axis cs:1750,0.790156634545292)
--(axis cs:2000,0.831851864172936)
--(axis cs:2250,0.831851864172936)
--(axis cs:2500,0.853749992495233)
--(axis cs:2750,0.858322915720337)
--(axis cs:3000,0.867375605442136)
--(axis cs:3000,0.892624385021121)
--(axis cs:3000,0.892624385021121)
--(axis cs:2750,0.891677084279663)
--(axis cs:2500,0.881249992007559)
--(axis cs:2250,0.865648126290321)
--(axis cs:2000,0.865648126290321)
--(axis cs:1750,0.852343348765407)
--(axis cs:1500,0.809738441018431)
--(axis cs:1250,0.769895592070889)
--(axis cs:1000,0.584208301925637)
--(axis cs:750,0.403288350092212)
--(axis cs:500,0.359677069968564)
--(axis cs:250,0.346614454193629)
--cycle;
\addlegendimage{area legend, fill=color0, fill opacity=0.2}
\addlegendentry{MetaRLBO}

\path [fill=color1, fill opacity=0.2]
(axis cs:250,0.346587166151618)
--(axis cs:250,0.300079500515048)
--(axis cs:500,0.372370396787671)
--(axis cs:750,0.41483958758355)
--(axis cs:1000,0.438987596630947)
--(axis cs:1250,0.44068338190776)
--(axis cs:1500,0.465771325680201)
--(axis cs:1750,0.489723106873799)
--(axis cs:2000,0.518240847660736)
--(axis cs:2250,0.531413876990699)
--(axis cs:2500,0.541782575342672)
--(axis cs:2750,0.554077267057695)
--(axis cs:3000,0.575662551675512)
--(axis cs:3000,0.647670781657821)
--(axis cs:3000,0.647670781657821)
--(axis cs:2750,0.629256066275638)
--(axis cs:2500,0.621550757990661)
--(axis cs:2250,0.608586123009301)
--(axis cs:2000,0.59842581900593)
--(axis cs:1750,0.576943559792867)
--(axis cs:1500,0.544228674319799)
--(axis cs:1250,0.522649951425573)
--(axis cs:1000,0.507679070035719)
--(axis cs:750,0.478493745749783)
--(axis cs:500,0.424296269878995)
--(axis cs:250,0.346587166151618)
--cycle;
\addlegendimage{area legend, fill=color1, fill opacity=0.2}
\addlegendentry{Adalead}

\path [fill=color2, fill opacity=0.2]
(axis cs:250,0.276370116691408)
--(axis cs:250,0.173629883308592)
--(axis cs:500,0.180502525316942)
--(axis cs:750,0.224293942020531)
--(axis cs:1000,0.230629960629941)
--(axis cs:1250,0.238714098238205)
--(axis cs:1500,0.246641422831204)
--(axis cs:1750,0.246641422831204)
--(axis cs:2000,0.246641422831204)
--(axis cs:2250,0.246641422831204)
--(axis cs:2500,0.246641422831204)
--(axis cs:2750,0.246641422831204)
--(axis cs:3000,0.246641422831204)
--(axis cs:3000,0.320025243835463)
--(axis cs:3000,0.320025243835463)
--(axis cs:2750,0.320025243835463)
--(axis cs:2500,0.320025243835463)
--(axis cs:2250,0.320025243835463)
--(axis cs:2000,0.320025243835463)
--(axis cs:1750,0.320025243835463)
--(axis cs:1500,0.320025243835463)
--(axis cs:1250,0.311285901761795)
--(axis cs:1000,0.309370039370059)
--(axis cs:750,0.302372724646135)
--(axis cs:500,0.279497474683058)
--(axis cs:250,0.276370116691408)
--cycle;
\addlegendimage{area legend, fill=color2, fill opacity=0.2}
\addlegendentry{Random}

\path [fill=color3, fill opacity=0.2]
(axis cs:250,0.249472187586535)
--(axis cs:250,0.227194479080131)
--(axis cs:500,0.27176013285204)
--(axis cs:750,0.340917517095361)
--(axis cs:1000,0.369125875719395)
--(axis cs:1250,0.388931687336871)
--(axis cs:1500,0.395857864376269)
--(axis cs:1750,0.406853599037414)
--(axis cs:2000,0.406853599037414)
--(axis cs:2250,0.421697562682992)
--(axis cs:2500,0.455)
--(axis cs:2750,0.455611678063574)
--(axis cs:3000,0.461591064971355)
--(axis cs:3000,0.498408935028645)
--(axis cs:3000,0.498408935028645)
--(axis cs:2750,0.461054988603092)
--(axis cs:2500,0.455)
--(axis cs:2250,0.451635770650342)
--(axis cs:2000,0.42647973429592)
--(axis cs:1750,0.42647973429592)
--(axis cs:1500,0.424142135623731)
--(axis cs:1250,0.417734979329795)
--(axis cs:1000,0.397540790947272)
--(axis cs:750,0.349082482904639)
--(axis cs:500,0.281573200481293)
--(axis cs:250,0.249472187586535)
--cycle;
\addlegendimage{area legend, fill=color3, fill opacity=0.2}
\addlegendentry{CMAES}

\path [fill=color4, fill opacity=0.2]
(axis cs:250,0.304888516028613)
--(axis cs:250,0.271778150638054)
--(axis cs:500,0.316081881462597)
--(axis cs:750,0.326010205144336)
--(axis cs:1000,0.343819486127799)
--(axis cs:1250,0.372135756428326)
--(axis cs:1500,0.387829587327927)
--(axis cs:1750,0.423581580757706)
--(axis cs:2000,0.465502525316942)
--(axis cs:2250,0.480559163211288)
--(axis cs:2500,0.499579599940899)
--(axis cs:2750,0.513171623173494)
--(axis cs:3000,0.572740274452388)
--(axis cs:3000,0.613926392214278)
--(axis cs:3000,0.613926392214278)
--(axis cs:2750,0.593495043493173)
--(axis cs:2500,0.577087066725767)
--(axis cs:2250,0.566107503455378)
--(axis cs:2000,0.564497474683058)
--(axis cs:1750,0.546418419242294)
--(axis cs:1500,0.518837079338739)
--(axis cs:1250,0.507864243571674)
--(axis cs:1000,0.459513847205534)
--(axis cs:750,0.423989794855664)
--(axis cs:500,0.40058478520407)
--(axis cs:250,0.304888516028613)
--cycle;
\addlegendimage{area legend, fill=color4, fill opacity=0.2}
\addlegendentry{Genetic}

\addplot [semithick, color0, forget plot]
table {%
250 0.336249999701977
500 0.354999996721745
750 0.391249999403954
1000 0.554999999701977
1250 0.747500002384186
1500 0.780000001192093
1750 0.82124999165535
2000 0.848749995231628
2250 0.848749995231628
2500 0.867499992251396
2750 0.875
3000 0.879999995231628
};
\addplot [semithick, color1, forget plot]
table {%
250 0.323333333333333
500 0.398333333333333
750 0.446666666666667
1000 0.473333333333333
1250 0.481666666666667
1500 0.505
1750 0.533333333333333
2000 0.558333333333333
2250 0.57
2500 0.581666666666667
2750 0.591666666666667
3000 0.611666666666667
};
\addplot [semithick, color2, forget plot]
table {%
250 0.225
500 0.23
750 0.263333333333333
1000 0.27
1250 0.275
1500 0.283333333333333
1750 0.283333333333333
2000 0.283333333333333
2250 0.283333333333333
2500 0.283333333333333
2750 0.283333333333333
3000 0.283333333333333
};
\addplot [semithick, color3, forget plot]
table {%
250 0.238333333333333
500 0.276666666666667
750 0.345
1000 0.383333333333333
1250 0.403333333333333
1500 0.41
1750 0.416666666666667
2000 0.416666666666667
2250 0.436666666666667
2500 0.455
2750 0.458333333333333
3000 0.48
};
\addplot [semithick, color4, forget plot]
table {%
250 0.288333333333333
500 0.358333333333333
750 0.375
1000 0.401666666666667
1250 0.44
1500 0.453333333333333
1750 0.485
2000 0.515
2250 0.523333333333333
2500 0.538333333333333
2750 0.553333333333333
3000 0.593333333333333
};
\end{axis}

\end{tikzpicture}

